Hy-DAT: A Tool to Address Hydropower Modeling Gaps Using Interdependency, Efficiency Curves, and Unit Dispatch Models

As the power system continues to be flooded with intermittent resources, it becomes more important to accurately assess the role of hydro and its impact on the power grid. While hydropower generation has been studied for decades, dependency of power generation on water availability and constraints in hydro operation are not well represented in power system models used in the planning and operation of large-scale interconnection studies. There are still multiple modeling gaps that need to be addressed; if not, they can lead to inaccurate operation and planning reliability studies, and consequently to unintentional load shedding or even blackouts. As a result, it is very important that hydropower is represented correctly in both steady-state and dynamic power system studies. In this paper, we discuss the development and use of the Hydrological Dispatch and Analysis Tool (Hy-DAT) as an interactive graphical user interface, that uses a novel methodology to address the hydropower modeling gaps like water availability and interdependency using a database and algorithms to generate accurate representative models for power system simulation.

==> sections/abstract.tex <==
As the power system continues to be flooded with 
intermittent resources, it becomes more important to 
accurately assess the role of hydro and its impact on the power 
grid. While hydropower generation has been studied for decades, 
dependency of power generation on water availability and 
constraints in hydro operation are not well represented in 
power system models used in the planning and operation of large-scale interconnection studies. There are still multiple modeling 
gaps that need to be addressed; if not, they can lead to 
inaccurate operation and planning reliability studies, and 
consequently to unintentional load shedding or even 
blackouts. As a result, it is very important that
hydropower is represented correctly in both steady-state and
dynamic power system studies. In this paper, a novel methodology is presented to address some of the hydropower modeling gaps like water availability and inter-dependency using a database, a set of tools and algorithms, and an interactive graphical user interface (GUI) to generate accurate representative models for power system simulation.

==> sections/conclusion.tex <==
\vspace{-1em}
\section{Concluding Remarks} \label{sec:con}

Operation and planning reliability studies do not consider 
environmental conditions and constraints such as water 
availability and interdependencies among power plants. The 
reason for such an approach is lack of coupling of hydro 
conditions and constraint with the electrical model used in 
power system planning and operation studies (power flow and 
dynamic models). Industry develops base cases for heavy 
winter and summer loading conditions as well as shoulder 
cases representing light loading conditions. In the environment 
of large renewable penetration of intermittent resources (solar 
and wind) and carbon-free goals, hydro becomes a more 
critical resource. For this reason, it is important to properly 
represent hydro conditions in base cases and, similar to 
developing cases having heavy and light load conditions, we 
need to have high and low hydro conditions properly 
represented in steady-state and dynamic models used for 
power system planning and operation reliability studies. This paper provides an end-to-end methodology for addressing modeling gaps in hydropower resources using a newly developed database and set of tools and algorithms to use historical data in accurately dispatching hydropower resources. 

==> sections/introduction.tex <==
\section{Introduction}
 In the evolving power system, where new renewable 
resources displace continually conventional generation and hydro 
becomes a single traditional resource that is fully controllable, it 
is timely to examine hydropower generation’s role in the power system 
of the future and its representation in power system operation 
and planning reliability studies. Energy generation through hydroelectricity has a vital role in the development of a region and its economy. Hydropower generation depends on a lot of external factors such as water availability due to annual precipitation and snow water melting as a result representing hydropower generation accurately in electrical power system models requires proper translation of hydrology into the electrical capability of the plants. As the renewable generation penetration continues to increase, hydropower operation has evolved from a base load resource to a regulating resource. As a result, it is very important that hydropower is represented correctly in both steady-state and dynamic power system studies \cite{mitra2023gaps}. These gaps in hydropower modeling are mainly a consequence of decoupling hydro conditions and hydro-based constraints with electrical models used in steady-state and dynamic studies. The 
following gaps have been identified in close collaboration 
with the industry:
\begin{itemize}
  \item Water availability in steady-state and dynamic models are not properly represented. 
\item Inter-dependencies among hydro projects in the same river systems are not properly represented. 
\item Environmental constraints are not represented in models. 
\item Rough zones are not represented in the power system 
model so generation dispatch in system studies might 
not be realistic. 
\item Many outdated dynamic models of hydropower generation 
turbines are still in use. 
\end{itemize}
In order to conduct more accurate planning and operation 
studies, and ensure the grid operates reliably, it is vital to more 
accurately model hydropower generation. In this paper, we present a methodology to address the hydropower modeling gaps with respect to water availability and inter-dependencies through the usage of databases and specific tools to translate historical hydrology into representative models that can be used in major power system simulations. The paper has the following sections: Section \ref{sec:db} provides the database components and features, Section \ref{sec:eff} provides an insight into the application of database for various tools like the  efficiency curve estimation, inter-dependency evaluation using historical datasets, and the regression mode used for unit-level dispatch of hydropower resources. Section \ref{sec:inter}  provides an integration of the various features for power system model updates. Finally, Section \ref{sec:con} concludes the paper.

==> sections/methodology.tex <==
\section{Methodology}
% To detect the electricity price spikes and analyze the underlying key drivers, we develop a comprehensive 
methods

==> tables/caiso_results.tex <==
\begin{table}[]
    \centering
    \caption{Caption}
    \label{tab:my_label}
    \ra{1.3}
    \resizebox{\columnwidth}{!}{\%
    \begin{tabular}{llll}
    \toprule
     \multirow[c]{7}{*}{Congestion (146, 60\%)} &  & \multirow[c]{2}{*}{PGAE (106, 43\%)} & Avg (4, 2\%)\\
     &  &  & Mov (104, 43\%)\\
     &  & \multirow[c]{2}{*}{SCE (54, 22\%)} & Avg (8, 3\%)\\
     &  &  & Mov (47, 19\%)\\
     &  & SDGE (6, 2\%) & Mov (6, 2\%)\\
     &  & \multirow[c]{2}{*}{VEA (120, 49\%)} & Avg (2, 1\%)\\
     &  &  & Mov (119, 49\%)\\  \hline
    \multirow[c]{2}{*}{Day Ahead (32, 13\%)} & Congestion (5, 2\%) & SCE (5, 2\%) & Avg (5, 2\%)\\
     & Energy (28, 11\%) & PGAE (28, 11\%) & Avg (28, 11\%)\\  \midrule
    Demand (13, 5\%) &  (13, 5\%) &  (13, 5\%) & Avg (13, 5\%)\\  \hline
    \multirow[c]{7}{*}{Forecasting Error (110, 45\%)} & \multirow[c]{5}{*}{Ver (99, 41\%)} & \multirow[c]{2}{*}{Dam (63, 26\%)} & Avg (16, 7\%)\\
     &  &  & Mov (51, 21\%)\\
     &  & Rtd (4, 2\%) & Avg (4, 2\%)\\
     &  & \multirow[c]{2}{*}{Rtpd (52, 21\%)} & Avg (14, 6\%)\\
     &  &  & Mov (41, 17\%)\\
     & \multirow[c]{2}{*}{Demand (21, 9\%)} & \multirow[c]{2}{*}{Dam (21, 9\%)} & Avg (12, 5\%)\\
     &  &  & Mov (9, 4\%)\\  \hline
    \multirow[c]{8}{*}{Generation (122, 50\%)} & \multirow[c]{2}{*}{Non-Renewables (24, 10\%)} & Nuclear (4, 2\%) & Mov (4, 2\%)\\
     &  & Thermal (20, 8\%) & Mov (20, 8\%)\\
     & \multirow[c]{6}{*}{Renewables (105, 43\%)} & \multirow[c]{2}{*}{Large.Hydro (64, 26\%)} & Avg (39, 16\%)\\
     &  &  & Mov (29, 12\%)\\
     &  & \multirow[c]{2}{*}{Non-Ver (16, 7\%)} & Avg (11, 5\%)\\
     &  &  & Mov (5, 2\%)\\
     &  & \multirow[c]{2}{*}{Ver (37, 15\%)} & Avg (24, 10\%)\\
     &  &  & Mov (13, 5\%)\\  \hline
    \multirow[c]{3}{*}{Regulation Prices (41, 17\%)} & \multirow[c]{3}{*}{ (41, 17\%)} & Rd (1, 0\%) & Avg (1, 0\%)\\
     &  & Rmd (1, 0\%) & Mov (1, 0\%)\\
     &  & Ru (40, 16\%) & Mov (40, 16\%)\\
     \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/data.tex <==
\begin{table}
    \centering
    \caption{Data Description}
    \label{tab:lodes}
    \scriptsize
    %\begin{tabular}{|l|p{2cm}|p{2cm}|p{2cm}|}
    \begin{tabular}{|p{1.5cm}|p{1.8cm}|p{1.75cm}|p{2cm}|}
    \toprule
    Parameter & Common Variables & CAISO & ISONE \\ [0.5ex] 
    \midrule
    Prices (P) &  Marginal Cost of Energy ($_{E}$), Marginal Cost of Congestion ($_{C}$) &  & \\ \midrule
    Generation (G) &  Nuclear ($_N$), Hydro ($_H$) & Thermal ($_T$), VER ($_{VER}$), Other Renewables ($_{OR}$) & Solar ($_S$), Wind ($_W$), Oil ($_O$), Landfill Gas ($_{LG}$), Refuse ($_R$), Wood ($_{Wo}$), Coal ($_C$), Natural Gas ($_{NG}$) \\\midrule
    Demand (D) & Load ($_L$) &  &  \\\midrule
    Forecast Error (FE) & Day-ahead demand ($_{D}$) & VER ($_{VER}$) & Wind ($_W$)\\\midrule
    Reserves (R) &  & Regulation Up ($_{RU}$), Regulation Down ($_{RD}$) &   \\\midrule
    Curtailment (C) &  & Wind ($_W$), Solar ($_S$) & \\\midrule
    Transfers ($T$) & Imports($_I$) & & Exports ($_E$)\\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/feature_count.tex <==
\begin{table}[ht!]
    \centering
    \caption{Feature Count: Derived (Raw)}
    \label{tab:lodes}
    % \scriptsize
    \resizebox{\columnwidth}{!}{%
    %\begin{tabular}{|l|p{2cm}|p{2cm}|p{2cm}|}
    \begin{tabular}{@{}l|cccccc@{}}
    \toprule
    Parameter & Prices & Generation & Demand & Forecast Error & Reserves & Others \\ [0.5ex]
    % \cmidrule{2-3} \cmidrule{5-6}
    % & Raw & Derived && Raw & Derived \\
    \midrule
    CAISO: 105(30) & 21(9) & 20(5) & 4(1) & 24(6) & 24(6) & 12(3) \\ \midrule
    ISO-NE: 170(56) & 53(26) & 40(10) & 4(1) & 9(3) & 56(14) & 8(2) \\
    \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/spike_summary.tex <==
\begin{table}[h!]
    \centering
    \caption{Spike Distribution}
    \label{tab:spike_distribution}
    \ra{1.3}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}l|cccccccccc@{}}
        \toprule
        ISO & \multicolumn{4}{c}{MCE ($\$$ per MW)} & \phantom{abc}& \multicolumn{5}{c}{Price Spike Events} \\
        \cmidrule{2-5} \cmidrule{7-11}
        & min & Q-95 & Q-99 & max && n & 2018 & 2019 & 2020 & 2021\\ 
        \midrule
        CAISO & -86.37 & 59.68 & 140.51 & 1152.71 && 1004 & 423 & 381 & 200 & - \\ 
        ISO-NE & -97.44 & 81.79 & 133.25 & 506.62 && 223 & - & - & 40 & 183 \\
        \bottomrule
    \end{tabular}
    }
\end{table}
